"We are at the mercy of others' opinion": Supporting Blind People in Recreational Window Shopping with AI-infused Technology

Engaging in recreational activities in public spaces poses challenges for blind people, often involving dependency on sighted help. Window shopping is a key recreational activity that remains inaccessible. In this paper, we investigate the information needs, challenges, and current approaches blind people have to recreational window shopping to inform the design of existing wayfinding and navigation technology for supporting blind shoppers in exploration and serendipitous discovery. We conduct a formative study with a total of 18 blind participants that include both focus groups (N=8) and interviews for requirements analysis (N=10). We find that there is a desire for push notifications of promotional information and pull notifications about shops of interest such as the targeted audience of a brand. Information about obstacles and points-of-interest required customization depending on one's mobility aid as well as presence of a crowd, children, and wheelchair users. We translate these findings into specific information modalities and rendering in the context of two existing AI-infused assistive applications: NavCog (a turn-by-turn navigation app) and Cabot (a navigation robot).

==> sections/notes.tex <==
- method: gender imbalance
- throughout: ai-infused 
- focus groups: joao on virtual nav
- focus groups: detecting pedestrians in crowded spaces, branham paper
- discussion (info requirements and design implications): kyungjun paper for recognition tech
- discussion (info requirements and design implications): generative ai description, narrative that is pleasing 
- discussion (smartphone apps): imove gesture recognition
- discussion (smartphone apps): generative ai information retrieval
- discussion (guide robots): addition of Towards Robotic Companions: Understanding Handler-Guide Dog Interactions for Informed Guide Dog Robot Design https://programs.sigchi.org/chi/2024/program/content/147890
- discussion (shopping services): addition of Navigating Real-World Challenges: A Quadruped Robot Guiding System for Visually Impaired People in Diverse Environments, https://programs.sigchi.org/chi/2024/program/content/147169





"I Don't Really Get Involved In That Way": Investigating Blind and Visually Impaired Individuals’ Experiences of Joint Attention with Sighted People
https://programs.sigchi.org/chi/2024/program/content/147896

% kameswaran2019cash,
% bradley2000study: purchase of clothing
% baker2002can: interview, those with visual impairments view the marketplace as a venue to fulfill task, recreational, and social needs, as well as to perform their expected roles. However, many visually impaired consumers may also regard the marketplace as a context in which to exercise-and relish-their independence
% swaine2014exploring: the mall's design for mobility or wayfinding, people with disabilities, interviews
% yu2015retail: retail layout, mobility is a challenge, focus groups,
% tullio2021you: their needs and experiences when navigating in shopping malls, mobility is a challenge, ethno

% One potential avenue for recreational window shopping for blind people lies in identifying design requirements that can augment these existing systems to better meet their unique needs and challenges. 

They have to rely on others' assistance to go shopping and come up with ways to cope with limited opportunities using online and offline platforms for independent exploration and window shopping. 

Expanding on their limited window shopping experiences, contributing to . 
Window shopping is not an activity that blind people can choose to engage themselves in due to the limitations to access information independently. It becomes mutually difficult for those providing and receiving assistance to communicate in the absence of specific needs for shopping:

% 

% what the store can do, need people who are trained to do, rather than substituting people - one way to gain information is to incorporate practices into the vendor sites


% information requirements, design implications, and potential applications for AI-infused technology to support recreational window shopping for blind people. The key findings are unique to the desirability and priority of information when exploring inside shopping malls. We also provide a deeper view of personal and situational needs that impact the design of informative notifications. 

% While our formative study is limited in its focus given a specific scenario (\ie, window shopping in indoor malls) that can impact the generalizability of our findings, we feel that our research strategy motivates supporting blind people in other exploration activities, whether indoor (\eg, airports) or outdoor (\eg, farmers markets). Research to encourage independent access to information for blind people and understand its requirements will be important for enhancing their recreational opportunities in both non-social and social settings. Future work will include further analysis of the impact of guidance systems developed based on our design implications to support real-world recreational activities for blind people. 


% future
% wayfinding and navigation systems






%  ~\cite{,McCarville2013Shopping,backstrom2006understanding} , shifting to online retailers and maintaining social distancing. 

% While we also see active areas of research in personal robot guidance systems which have great potential in helping blind users in recreational shopping through autonomous navigation, obstacle avoidance, and information feedback of their surroundings~\cite{guerreiro2019cabot,tobita2017examination,lacey2000context,kulyukin2005robocart}, no discussion has been made to apply the design of advanced guidance systems for blind window shoppers. Though barriers to engage in window shopping go beyond navigation issues, a potential solution is to extend existing assistive technologies that ensure their navigation, while supporting their serendipitous discovery of new, desirable information to enjoy blind window shopping.

We have seen many innovations in navigation technology, including smaller, more accurate location-based applications and access to information above and beyond turn-by-turn directions. 

We can apply these navigation robot technologies for recreational shopping that the users can concentrate on information to enjoy window shopping without worrying about their mobility.

% We are specifically targeting a window shopping scenario in recreational shopping. Working towards this goal, it is important to understand their information needs, challenges, and current approaches people with visual impairments have to window shopping. Due to their daily challenges in mobility and information access, they must depend on the assistance of other sighted shopping companions or store associates to engage in in-person shopping, although it doesn't always result in proper accommodation or satisfactory experiences for their needs~\cite{yu2015retail}. 

% Window shopping provides a new lens to discuss information requirements which might fall differently from the previous work that investigated and provided solutions for their navigation~\cite{dakopoulos2009wearable,faccanha2020om,hub2003design} or grocery shopping needs~\cite{boldu2018fingerreader2,lee2017reaching,lanigan2006trinetra,szpiro2016finding}. 

Public environments provide opportunities and means for various types of recreation. People can spend their leisure time playing sports at neighborhood parks or fitness centers, visiting museums or sports events, going shopping, or dining out with friends. Recreation is an important factor that affects the quality of life for many individuals, as it provides social interaction as well as physical and emotional health benefits~\cite{barnett2008perceived, tsai2005cross, iso1996leisure}.

Shopping malls have once been popular entertainment and social venues for such recreational shoppers~\cite{el2013shopping,bloch1991leisure,farrag2010mall}. However, prior research in marketing focusing on consumers with disabilities have acknowledged that, despite the growing infrastructure of e-commerce, they hold additional meanings to be able to shop in stores, which include formulating a sense of ``I am here'' and `` I belong'' in the community for people with visual impairments~\cite{baker2006consumer} and facilitating equal participation as an active agent in the marketplace~\cite{elms2012consumer}.

Shopping malls have also been analyzed as entertainment venues composed of promotional areas, relaxation spaces, and social use areas~\cite{el2013shopping,farrag2010mall}. 

Other scholars also see hope for a post-pandemic retail renaissance~\cite{danziger2020malls, weintraub2020future}.

%1) push notification of visual description (e.g., window displays) is desirable to fill , 2) pull notification of detailed information (e.g., promotion, general fashion styles or items carried) is preferred for the shops of their interest, and 3) alerts for obstacles and points of interest need customization . 

% Though our focus is people with vision impairments and their specific technology needs to reinvent their recreational shopping experiences, our findings support universal design approaches, as accessibility of services and information affect everyone. Our main contribution, however, is a description of how information requirements are influenced by the wide range of personality and situational characteristics (e.g. just a day for walking around, have a drink cup and want to throw it away, want to know landmarks for meeting people).

% To gain better insights about their shopping experiences, focus groups discovered how people with visual impairments perform in-person shopping as a recreational activity, analyzed in the context of their shopping strategies and challenges. 

To increase recreational shopping opportunities for people with visual impairments, we discuss use cases to extend existing assistive technologies, such as in smartphone-based, robot-based, or virtual guidance systems.

%The authors explored the information needs, challenges, and current approaches people with vision impairments have to window shopping. They used focus groups and one-on-one interviews centered around the imagined experience of being lead by a navigation robot to explore these ideas. This is important work in the space of blind and low vision shopping and travel experience that works beyond point-to-point navigation. extend the applicability of existing mobile systems designed for wayfinding and safe travel experience. novel insights such as the importance of describing window displays to get a feel for the store's aesthetic and the season's style.

here are often barriers to blind people's engagement in the community and are susceptible to disruption of their mental health and well-being~\cite{honey2011mental,mithen2015inequalities,emerson2021loneliness}.

This research addresses the problem concerning the blind and low vision community in that they have no equal opportunity to engage themselves in recreational activities without being dependent on sighted people. 
% Participation in recreational activities positively impacts the health of individuals~\cite{}. Equal access to services and information is essential to ensure physical, cognitive, and emotional well-being of people with disabilities. with an increasing concern on its accessibility of services and information for people with visual impairments. 

% GPS-based localization is also used outdoors~\cite{yelamarthi2010rfid, mori1998robotic}, but accuracy remains a challenge. Recent research efforts have been made to promote robot guidance systems for blind people navigating in indoor environments~\cite{}. Kulyukin [22, 23] presented a robot guide that helped blind people wayfind indoors with RFID tags in the environment. The user of Kulyukin’s robot guide system held the robot with a dog leash in addition to their mobility aid, receiving audio and tactile feedback. This work motivates ours: researchers believe that robots would be effective tools for indoor navigation, but they paid little to no attention to the design of the human-robot interaction.

%~\cite{paladugu2013supporting,jafri2014gps}to PVI in outdoor [29] and indoor [37] environments


% Much of the current effort has utilized location-based smartphone apps, allowing users to listen to audio content of nearby artworks~\cite{gonzalez2017path,rector2017eyes} and receive continuous navigation assistance inside a museum~\cite{meliones2018blind,asakawa2019independent}. 

% mobility - obstacle avoidance - robot users, (search/pre-set, want to know about pedestrians even if they are guided around

% , guiding users to a destination and informing them of relevant points-of-interest (POIs)~\cite{sato2017navcog3,cheraghi2017guidebeacon,ran2004drishti,BlindSquare}. Many wearable devices have been introduced to support detection and warning of obstacles~\cite{dakopoulos2009wearable,katzschmann2018safe,li2016isana,rodriguez2012assisting}, as well as for effective search of products in grocery shopping~\cite{boldu2018fingerreader2,lee2017reaching,zhao2016cuesee}. 

%El Hedhli~\textit{et al.}~\cite{el2013shopping} argue that shopping goes beyond consumer life of acquiring material goods and contributes to people's satisfaction in important life domains (social, leisure, and community life).

We aim to address the limited opportunities . Window shopping provides a new lens to design future guidance systems, with requirements falling differently from systems tailored to navigation~\cite{dakopoulos2009wearable,faccanha2020om,hub2003design} or grocery shopping needs~\cite{boldu2018fingerreader2,lanigan2006trinetra,szpiro2016finding}. We want to build an understanding of potential directions for technology to encourage equal opportunities for independent recreational experiences. 

Accessible shopping for blind people has been explored in the space of assistive technologies \eg, enabling search and location of specific items and overall wayfinding in the store. This research pays particular attention to the barriers that can exist in new shopping experiences beyond point-to-point navigation -- ~\textit{window shopping} used for recreational purposes

 With window shopping often taking the form of serendipitous discovery of previously unknown information (\eg, new fashion trends, sale items),


Perhaps this reflects the work examining the shopping practices of blind people, which are deemed to carry additional meanings beyond just acquiring goods~\cite{baker2006consumer,yu2015retail}---\eg, formulating a sense of ``I am here'' and `` I belong'' in the community~\cite{baker2006consumer}.

% More so, building this sense of community is particularly relevant for shopping malls and retail stores as we navigate the post-pandemic landscape~\cite{weintraub2020future,reese2020integrating}. 

Informing blind users about POIs and accessibility issues is helpful in acquiring visual cues if they are using or looking for elevators, stairs, restrooms, or food courts in shopping malls. Another advantageous situation is inside a large airport. As highlighted by Guerreiro \etal~\cite{guerreiro2019airport}, blind individuals can receive guidance to their target gate but have no opportunity to explore shops or restaurants. 

What kind of information do blind users want to hear about shops that usually offer visual stimulation to attract customers for enjoyable shopping experiences? What are the relevant POIs in recreational shopping? Similar to receiving alerts from wearable obstacle systems, do they want to be informed about approaching obstacles (e.g., pedestrians) even when they are physically guided by the robot? We aim to answer such questions.
participants who are cane users had different views on building awareness of their surroundings


% Participants outlined a set of notifications to gain awareness of the mall environment; some of them were obstacles to avoid and others were POIs that help them build a mental map of the surrounding area while moving. 


K p3
A p2
H p4
N p1 dog

C p6
M p7
V p8 cane
S p5

Given the scenario of window shopping in a mall with a guide robot, a different group of 10 participants was prompted with a list of features (as highlighted in Section~\ref{features}) to provide feedback on whether and how they would prefer accessing relevant information and identify any missing features from the list. 
% They discussed the types of information that they would like to hear with regards to shops in the mall, as well as the surrounding environment including nearby POIs and obstacles.

where they can customize their information preferences beforehand. As desirability of notifications about obstacles and POIs varied among participants depending on their mobility aids or situations, having a setting to control O\&M preferences was also pointed out by P13: 

 we see an opportunity to implement these features e.g., by combining large language models with real-time search [] or augmenting them with knowledge bases []


 we first gain insights into window-shopping challenges and opportunities and identify a set of information needs. Then, we set up  to assess the types of notifications blind people prefer grounded in a simulated scenario of wayfinding and navigation systems for recreational window shopping. 

 % While our formative study is limited in scope to this specific scenario, potentially affecting the generalizability of our findings, we believe that our research strategy provides a compelling framework for supporting blind people in a variety of exploration activities, whether indoors (\eg, airports) or outdoors (\eg, farmers markets). Understanding their unique requirements is crucial for enhancing their recreational opportunities. 

